Global vs. s-t Vertex Connectivity Beyond Sequential: Almost-Perfect Reductions & Near-Optimal Separations

A recent breakthrough by [LNPSY STOC'21] showed that solving s-t vertex connectivity is sufficient (up to polylogarithmic factors) to solve (global) vertex connectivity in the sequential model. This raises a natural question: What is the relationship between s-t and global vertex connectivity in other computational models? In this paper, we demonstrate that the connection between global and s-t variants behaves very differently across computational models: 1.In parallel and distributed models, we obtain almost tight reductions from global to s-t vertex connectivity. In PRAM, this leads to a $n^{\omega+o(1)}$-work and $n^{o(1)}$-depth algorithm for vertex connectivity, improving over the 35-year-old $\tilde O(n^{\omega+1})$-work $O(\log^2n)$-depth algorithm by [LLW FOCS'86], where $\omega$ is the matrix multiplication exponent and $n$ is the number of vertices. In CONGEST, the reduction implies the first sublinear-round (when the diameter is moderately small) vertex connectivity algorithm. This answers an open question in [JM STOC'23]. 2. In contrast, we show that global vertex connectivity is strictly harder than s-t vertex connectivity in the two-party communication setting, requiring $\tilde \Theta (n^{1.5})$ bits of communication. The s-t variant was known to be solvable in $\tilde O(n)$ communication [BvdBEMN FOCS'22]. Our results resolve open problems raised by [MN STOC'20, BvdBEMN FOCS'22, AS SOSA'23]. At the heart of our results is a new graph decomposition framework we call \emph{common-neighborhood clustering}, which can be applied in multiple models. Finally, we observe that global vertex connectivity cannot be solved without using s-t vertex connectivity, by proving an s-t to global reduction in dense graphs, in the PRAM and communication models.

==> Distributed.tex <==


\section{A Distributed Algorithm in \congest Model} \label{sec:congest alg}


We prove \Cref{thm:congest} in this section. Let $G = (V,E)$ be an input graph. Let $V_{\textlow} := \{ v \in V \colon \textdeg_G(v) \leq 10\kappa_G\}$. For any vertex set $U \subseteq V$ , we define $U_{\textlow} := U \cap V_{\textlow}$.

\begin{lemma} [Using communication algorithm] \label{lem:using communication}
    There is a distributed algorithm running on an $n$-vertex undirected graph $G$ with diameter $D$ that takes parameters  $\tau$, and  outputs  a separator $S'$ in $\tilde O(( \tau + n + \sqrt{D})n^{o(1)} )$ rounds. In addition, if there is a vertex mincut $(L,S,R)$ where $|R| \geq |L|$ satisfying
     \begin{align} \label{eq:k-scratch}
          |L| \leq \tau, |L|  \leq  0.01|S| \text{ and } |S_{\textlow}| \geq 10 \cdot |L|\log^2n,
     \end{align}
    then $S'$ is a minimum separator with high probability.
\end{lemma}



If a vertex mincut violates \Cref{eq:k-scratch}, then we will use the distributed isolating cut lemma.  Let $T_{\textbm}(n,D)$ be the number of rounds needed to compute a subgraph maximum bipartite matching on a graph with $n$ vertices and diameter $D$.


\begin{lemma} [Using distributed isolating cut lemma] \label{lem:using dist isolating cut lemma}
    There is a distributed algorithm running on an $n$-vertex undirected graph $G$ with diameter $D$ and outputs a separator $S'$ in $\tilde O(\sqrt{n\cdot  T_{\textbm}(n,D)})$ rounds. In addition, if there is a vertex mincut $(L,S,R)$ where $|R| \geq |L|$ that
      \begin{align} \label{eq:k-nonscratch}
         |L| \leq  0.01|S| \text{ and } |S_{\textlow}| < 10 \cdot |L|\log^2n
     \end{align}
      or,
      \begin{align} \label{eq:k-Llarge}
         |L| >  0.01|S|
     \end{align}
     then $S'$ is a minimum separator with high probability.
\end{lemma}

We are now ready to prove \Cref{thm:congest}.
\begin{proof}[Proof of \Cref{thm:congest}]
First, we compute $S_1$ obtained from \Cref{lem:using dist isolating cut lemma} in  $\tilde O(\sqrt{n\cdot  T_{\textbm}(n,D)})$ rounds. Let $(L,S,R)$ be a vertex mincut (WLOG, $|R| \geq |L|$). If it satisfies \Cref{eq:k-nonscratch} or \Cref{eq:k-Llarge}, then $S_1$ is a minimum separator and we are done. Now, we assume that
$$ |L| \leq 0.01|S|,  |S_{\textlow}| \geq 10 |L| \log^2n.$$
Let $\tau$ be a parameter to be chosen. We compute a separator $S_2$ from \Cref{lem:using communication} with parameter $\tau$. If $(L,S,R)$ satisfies \Cref{eq:k-scratch}, then $S_2$ is a minimum separator and we are done.  The remaining case is
$ |L| \geq \tau.$ To handle this case, we sample $ \lceil 100 \frac{n}{\tau} \log n \rceil$ vertices $X$ and for each sample $x \in X$, we sample $y_1,\ldots, y_{O(\log n)}$ non-neighbors of $x$, compute $(x,y_i)$-vertex mincut for all $i$, and take the minimum separators among all of them.  We show that this algorithm will output a minimum separator with high probability. Since we sample $\lceil 100 \frac{n}{\tau} \log n \rceil$ vertices and $|L| \geq \tau$, there is a vertex $x \in L$ with high probability. Assume $x \in L$.  It is enough to show that we obtain a non-neighbor of $x$, denoted by $y \in R$. Let $\texttt{NN}(x)$ as the set of non-neighbors of $x$ in $G$. Since $N(x) \subseteq L \cup S$ and $|N(x)| \geq |S|$, we have
\begin{align}\label{eq:nnx small}
    |\texttt{NN}(x) \cap (L\cup S)| \leq |L|.
\end{align}
So given $x \in L$, the probability that a random non-neighbor of $x$ is in $R$ is $ \frac{|R|}{|\texttt{NN(x)}|} \overset{(\ref{eq:nnx small})}{\geq} \frac{|R|}{|L|+|R|} \geq 1/2.$  Therefore, one of non-neighbors $y_i \in R$ with high probability, and we are done.  The running time for the last two algorithms is $\tilde O( (\sqrt{n} + D + \tau)n^{o(1)} + \frac{n}{\tau} \cdot T_{\textbm}(n,D))$. By selecting $\tau = \sqrt{n\cdot  T_{\textbm}(n,D)}$, we obtain the desired running time.
\end{proof}

\subsection{Using the Communication Algorithm}  \label{sec:using communication congest}


\begin{algorithm}
	\caption{FindUnbalanced($G,\tau$)}\label{alg:unbal congest}
	\KwData{A graph $G=(V,E)$, a number $\tau < n$.}
	\KwResult{A separator $S$.}
	\For{$i=1,2,...,\lceil\log \tau \rceil$}{
		$\ell\leftarrow 2^i$\;
		Each vertex $u$ compute $\sk{\ell}(A_u)$ using~\Cref{lem:sketching}.\;
            Each vertex $u$ sends a token $(u,\sk{\ell}(A_u))$ to all its neighbors.\;\label{line:send token to all neighbors}

            Let $\gamma(n)$ be the function in the $n^{o(1)}$ term described in \Cref{lem:snccorrectness}(2).\;

		\Repeat{$\gamma(n) \cdot \lceil 100\log n \rceil$ \normalfont{times} }{ \label{line:repeat cluster}
             Apply \Cref{lem:snccongest} with parameter $\ell$ to obtain the sparse neighborhood cover $\mathcal{C}_{\ell}$\; \label{line:run snc in congest}
             \Repeat{$\lceil 1000\log n \rceil$ \normalfont{times}}{
                Run the following in parallel.\;
			\ForEach{\normalfont{cluster} $C \in \mathcal{C}_{\ell}$}{
                 	\ForEach{\normalfont{vertex} $v \in N_G(C) \cup C$}{
                Shuffle the set of tokens received from all vertices in $C \cap N_G(v)$ and send each token to each node in $C \cap N_G(v)$. More precisely,  Let $f: C \cap N_G(v) \rightarrow C \cap N_G(v)$ be a uniformly random bijective mapping. For each node $w \in C \cap N_G(v)$, $v$ sends the token received from $w$ at \Cref{line:send token to all neighbors} to $f(w)$. \;\label{line6}
                        }

            }
			}
		}
		\ForEach{$u\in V$}{
		    Let $V'$ contain all nodes $v$ where $u$ received the token $(v,\sk{\ell}(A_v))$ and $\SpaRec{}(\sk{\ell}(A_u),\sk{\ell}(A_v))\not=\bot$\;
                Find $A_v$ for any $v\in V'$ by using $\SpaRec{}$ and $A_u$\;
                Find $L_u\subseteq V'$ with the smallest $|N_G(L_u)|$ with $|N_G(L_u)|+|L_u|<n$\;
		}
	}
        Find $u\in V$ with the smallest $|N_G(L_u)|$ denoted as $u^*$\;
        Let $u_{\min}$ be a min-degree node\;
	\Return{$N_G(L_{u^*})$} or $N_G(u_{\min})$ if $u^*$ does not exist.
\end{algorithm}

We prove \Cref{lem:using communication} in this section. We present the algorithm and analysis.  For any vertex $v$, we denote $A_v$ as a vector of the neighbors of $v$ from the adjacency matrix $A$ representation of graph $G$.   The main goal is to ensure that any vertex $u \in L$ learns the sketch $\sk{\ell}(A_v)$ for all $v \in L$ (when $|L|$ is estimated by $\ell$ within a factor of 2).  We will do this using the sparse neighborhood cover.  The algorithm is depicted in \Cref{alg:unbal congest}.


\paragraph{Running Time.} We prove that \Cref{alg:unbal congest} runs in $\tOh{ (\tau + \sqrt{n}+D)n^{o(1)}}$ rounds. Fix $i$ in the outer loop. First, each token in~\cref{line:send token to all neighbors} needs $\tOh{\ell} = \tOh{\tau}$ rounds to send. In \Cref{line:run snc in congest}, it takes $\tOh{\sqrt{n}+D}$ rounds to run sparse neighborhood cover. The entire loop of \Cref{line:repeat cluster} can be implemented in $\tOh{ (\sqrt{n}+D+\ell)n^{o(1)}}$ rounds because each node can belong to $O(\log^2 n)$ clusters (\Cref{lem:snccongest}), and we repeat for $O(\gamma \log^2 n) = n^{o(1)}$ iterations.  The rest of the loop can be done locally without communication. Finally, aggregating the information about global mincut can be done in $O(\sqrt{n}+D)$ time.


\paragraph{Correctness.}  Let $S^*$ be the separator returned by \Cref{alg:unbal congest}. According to~\cref{lem:sketching}, each vertex $u$ gets the correct information about $A_v$ for any $v\in V'$. Thus, $N_G(L_u)$ must be a valid cut w.h.p. since $|N_G(L_u)|+|L_u|<n$.

We prove that $S^*$ is a vertex mincut w.h.p. if $G$ contains a vertex mincut $(L,S,R)$ satisfying \Cref{eq:k-scratch}. Suppose $G$ contains such a cut $(L,S,R)$.  There must exist iteration $i$ such that $|L|\le \ell\le 2|L|$. We focus on this iteration. Let $u$ be an arbitrary node in $L$. We will prove that $u$ will receive tokens $(v,\sk{\ell}(A_v))$ from any $v\in L$ with high probability. If true, then by union bounds we have $L\subseteq V'$, and thus $|N(L_u)| \leq |S| = \kappa_G$.


In the analysis, we will use the following properties of the sparse neighborhood cover described in \Cref{lem:snccongest}.

\begin{lemma} \label{lem:C small if contains L} For any cluster $C \in \mathcal{C}_{\ell}$ from the sparse neighborhood cover from \Cref{lem:snccongest} with parameter $\ell \in [|L|, 2|L|]$, if $L \subseteq C$, then $|C| \leq 20|S|$ with high probability.
\end{lemma}
\begin{proof}
    Let $u \in L \subseteq C$. Since all but $|L|$ neighbors of $u$ must be in $S$, we have $|N_G(u) \cap S_{\textlow}| \geq |S_{\textlow}| - |L|$. By low diameter property of the cluster (\Cref{lem:snccongest}), for all $w \in C$, we have $|N_G(u) \triangle N_G(w)| = O(\ell\log n) = O(|L|\log n)$ with high probability, and thus
    $$|N_G(w) \cap S_{\textlow}| \geq |S_{\textlow}| - O(|L|\log n) \overset{(\ref{eq:k-scratch})}{\geq} |S_{\textlow}|/2.$$
    That is, each $w \in C$ has at least $|S_{\textlow}|/2$ neighbors in $S_{\textlow}$. On the other hand, each $v \in S_{\textlow}$ has degree at most $10\kappa = 10|S|$. Therefore,
    $$ |C| \cdot |S_{\textlow}|/2 \leq |E_G(S_{\textlow},V)| \leq 10|S||S_{\textlow}|.$$
    We conclude that $|C| \leq 20|S|$ with high probability.
\end{proof}


Since we run sparse neighborhood cover for $O(\gamma \cdot \log n)$ iterations, by \Cref{lem:snccongest}, there is an iteration of the sparse neighborhood cover $\mathcal{C}_{\ell}$ such that $L \subseteq C \in \mathcal{C_{\ell}}$ with high probability. We now fix such a cluster $C$ for analysis.
\begin{claim} \label{claim:common neighbors in cluster}
    For any vertex $v \in L$, $N_G(u) \cap N_G(v) \subseteq C \cup N_G(C)$ and $|N_G(u) \cap N_G(v)| \geq 0.9|S|$.
\end{claim}
\begin{proof}
Since $L \subseteq C$, $N_G(u) \cap N_G(v) \subseteq C \cup N_G(C)$. Observe that any vertex $v$ must have at least $|S|$ neighbors (otherwise, $S$ is not a vertex mincut). Since $u,v \in L$, we have $|N_G(u) \cap N_G(v)| \geq |S| - 2|L| \overset{(\ref{eq:k-scratch})}{\geq} 0.9|S|.$
\end{proof}

Fix $v \in L$, we next compute the probability that $u$ receives a token $(v,\sk{\ell}(A_v))$ from $v$. By \Cref{claim:common neighbors in cluster}, $u$ can receive the token   $(v,\sk{\ell}(A_v))$ from their common neighbors $N_G(u) \cap N_G(v)$ which are in $C \cup N_G(C)$. For any node $w \in N_G(u) \cap N_G(v) \subseteq C \cup N_G(C)$, by design, $w$ shuffles the tokens received from $N_G(w) \cap C$ (at \Cref{line:send token to all neighbors}) and sends each token to every node in $N_G(w) \cap C$. So, in this iteration, $u$ receives the token $(v,\sk{\ell}(A_v))$ from $w \in N_G(u) \cap N_G(v)$  with probability at least $1/|C|$. Therefore, the probability that $u$ does not receive the token $(v,\sk{\ell}(A_v))$ is at most

$$  \left(1-\frac{1}{|C|}\right)^{|N_G(u) \cap N_G(v)| 1000 \log n} \le \left(1-\frac{1}{20|S|}\right)^{900|S|\log n}\le \frac{1}{n^{10}}. $$
The first inequality follows from \Cref{claim:common neighbors in cluster} and \Cref{lem:C small if contains L}.








\subsection {Using Distributed Isolating Cut Lemma} \label{sec:using isolating cut congest}

We prove \Cref{lem:using dist isolating cut lemma} in this section. We denote $\delta(G)$ as the minimum degree of vertices in $G$. For a vertex set $A\subseteq V$, $G[A]$ is the induced subgraph of $G$ on $A$.
Let $T$ be an independent set. We say that a vertex cut $S$ is $t$-\textit{isolating} for some $t \in T$ if $S$ is an $(t,T-\{t\})$-vertex cut. We say that $S$ is $t$-\textit{isolating vertex mincut} if $S$ is a $t$-isolating vertex cut of minimum size.

\begin{lemma} [Distributed Isolating Cut Lemma] \label{lem:isolating cut congest}
    There is a distributed algorithm, denoted as $\textsc{MinIsolatingVC(G,T)}$, running on a graph $G = (V,E)$ with an independent set $T \subseteq V$ of size at least 2, that returns a vertex cut that is the minimum over all $t$-isolating vertex mincut. The algorithm runs in $\tilde O(\sqrt{n\cdot T_{\textbm}(n,D)})$ rounds.
\end{lemma}

We prove \Cref{lem:isolating cut congest} in \Cref{sec:isolating cut congest}. We now prove \Cref{lem:using dist isolating cut lemma}. We will describe an algorithm that always outputs a valid cut. The goal is to find a vertex set that is \textit{isolated} by the vertex mincut $(L,S,R)$. Let $T \subseteq V$ be a vertex set in $G = (V,E)$. We say that $(L,S,R)$ \textit{isolates} $T$ if  $|L \cap T| =1, |T \cap S| = 0, |T \cap R| \geq 1$. Given a vertex set isolated by a vertex mincut, we can compute a minimum separator using the isolating cut lemma.

\begin{claim} \label{claim:isolate then done}
    If $T$ is isolated by $(L,S,R)$ and $T'$ is a maximal independent set of $T$, then $\textsc{MinIsolatingVC}(G,T')$ returns a minimum separator.
\end{claim}
\begin{proof}
By definition, $T'$ is also isolated by $(L,S,R)$. Let $t \in L \cap T$ be the unique vertex in $L \cap T$. So, $T' - \{t\} \subseteq R$, and thus a $(t,T' -\{t\})$-min-separator has size at most $|S|$.  By \Cref{lem:isolating cut congest}, $\textsc{MinIsolatingVC}(G,T')$ returns a cut of size at most the size of a $(t,T' -\{t\})$-min-separator which is at most $|S|$, and we are done.
\end{proof}


We are now ready to prove \Cref{lem:using dist isolating cut lemma}. We present the algorithm and analysis.

\paragraph{Algorithm.} The algorithm runs on graph $G = (V,E)$.  Repeat for $\lceil 100 \log^5 n \rceil$ times:
\begin{enumerate}
    \item Let $\ell^{(i)} := 2^i$ for each $i =1,2,\ldots, \lceil \log n \rceil$, and let  $r$ be a random vertex.
    \item For each $i$,
     \begin{enumerate}
         \item Let $T_i^{\textlow}$  be a set obtained by selecting each vertex in $V_{\textlow}$ with probability $1/\ell^{(i)}$.
         \item Let $T_{i}$  be a set obtained by selecting each vertex in $V$ with probability $1/\ell^{(i)}$.
         \item let $\mathcal{T} := \{T_{i}^{\textlow}, T_i, T_{i}^{\textlow} \cup \{r\}, T_i \cup \{r\}\} $ and for all $T \in \mathcal{T}$, run $\textsc{MinIsolatingVC}(G,I(T))$ where $I(T)$ is an arbitrary maximal independent set of $T$.
     \end{enumerate}
\end{enumerate}
\textbf{Return} the smallest among cuts found in Step 4 or the min-degree vertex cut, whichever is smaller.


\paragraph{Running time.} It takes $\tilde O(\sqrt{n \cdot T_{\textbm}(n,D)})$ rounds because the number of calls to $\textsc{MinIsolatingVC}(G,T)$ is $O(\log^5 n)$.


\paragraph{Correctness.} The algorithm returns a valid cut by design. We prove that if a vertex mincut $(L,S,R)$ satisies \Cref{eq:k-nonscratch} or \Cref{eq:k-Llarge}, then the algorithm produces a terminal set $T \subseteq V$ isolated by $(L,S,R)$ with probability at least $\Omega(1/\log^4n)$. If true, then \Cref{claim:isolate then done} implies that we obtain a vertex mincut with high probability (since we repeat for $\lceil 100 \log^5n \rceil$ times).

We first consider the case $(L,S,R)$ satisfies \Cref{eq:k-nonscratch}. In this case, $L \subseteq V_{\textlow}$ since every node $v \in L$ has degree at most $|L| +|S| \overset{(\ref{eq:k-nonscratch})}{\leq} 1.01|S| \leq 2|S| = 2\kappa$. So we have $L_{\textlow} := L \cap V_{\textlow} = L$. There is iteration $i$ such that $\ell_i \in [|L_{\textlow}|+|S_{\textlow}|, 2(|L|+|S_{\textlow}|)]$. Denote $p = 1/\ell_i$. Next, we observe the property in $R$.
\begin{itemize}
    \item If $|S| < n/10$, then $|R| = n - |L| - |S| \geq 0.3n$, then $r \in R$ with a constant probability.   Therefore, the probability that $(L,S,R)$ isolates $T := T_i^{\textlow} \cup \{r\}$ is  at least
    \begin{align*}
        \mathbb{P}(|T \cap L_{\textlow}| = 1, T \cap S_{\textlow} = \emptyset, r\in R) &= |L|p(1-p)^{|L|-1} \cdot (1-p)^{|S_{\textlow}|} \cdot \Omega(1) \\
        &= \Omega(|L|p (1-p)^{|L|+|S_{\textlow}|-1}) \\
        &= \Omega(1/\log ^2n).
    \end{align*}
    The last equality follows since  $|L|p = \Omega(\frac{|L|}{|L|+|S_{\textlow}|}) \overset{(\ref{eq:k-nonscratch})}{=} \Omega(\frac{1}{\log^2 n})$ and $p = \Theta(\frac{1}{|L|+|S_{\textlow}|})$.
    \item If $|S| \geq n/10$, then $V = V_{\textlow}$ because every node has degree at most $n-1 \leq 10|S| = 10 \kappa$.   Therefore, the probability that $(L,S,R)$ isolates $T := T_i^{\textlow}$ is  at least
       \begin{align*}
        \mathbb{P}(|T \cap L_{\textlow}| = 1, T \cap S_{\textlow} = \emptyset, |T \cap R_{\textlow}| \geq 1)
        &\geq   \mathbb{P}(|T \cap L_{\textlow}| = 1)^2 \mathbb{P}(T \cap S_{\textlow} = \emptyset)\\
        &\geq (|L|p)^2(1-p)^{2|L|-2} \cdot (1-p)^{|S_{\textlow}|}\\
        &= \Omega((|L|p)^2 (1-p)^{2|L|+|S_{\textlow}|-2}) \\
        &= \Omega(1/\log ^4n).
    \end{align*}
\end{itemize}

Finally, for the case $|L| > 0.01|S|$ we can show that the probability that $(L,S,R)$ isolates $T_i$ or $T_i \cup \{r\}$ is $\Omega(1)$ using the same calculation and we omit it for brevity.


\subsection{Distributed Isolating Cut Lemma for \congest} \label{sec:isolating cut congest}

We prove \Cref{lem:isolating cut congest} in this section.  We first review an algorithm for the isolating cut lemma~\cite{LiNPSY21} in the sequential model.

\paragraph{Algorithm (Sequential).} The inputs consist of the input graph $G = (V,E)$ and an independent set $T \subseteq V$ of size at least $2$.
\begin{enumerate}
    \item Encode each $t \in T$ as a binary string of length $\ceil{\log_2|T|}$. For each $i \leq  \ceil{\log_2|T|}$, define       $A_i :=  \{ t \in T \colon i^{\text{th}} \text{bit of }  $t $ = 0 \}$ and   $B_i := T - A_i$
    Compute $F_i := (A_i,B_i)$-vertex mincut.
    \item For each $s \in T$, compute a connected component containing $s$, denoted by $U_s$, in $G - \bigcup_iF_i$.
    \item For each $s \in T$, define $G'_s$ as $G[N_G[U_s]]$ followed by (1) adding an additional vertex $t$ and all edges from $t$ to $N_G(U_s)$, and (2) remove all edges inside $N_G(U_s)$. Then, compute a minimum $(s,t)$-separator denoted by $C_s$ in $G'_s$.
\end{enumerate}

We summarize the correctness into the following lemma.
\begin{lemma} [\cite{LiNPSY21}]
For each  $s \in T$, $C_s$ is an $(s, T - \{s\})$-min-separator in $G$.
\end{lemma}

In the distributed setting, the first two steps can be implemented in  $O(\log |T|)$ calls of a bipartite maximum matching.
 However, there are two issues to implement the third step. First, the additional vertex $t$ can be viewed as a contraction of $V - N_G[U_s]$ into a single vertex, which is a global operation. For distributed implementation, we need the graph to be local.  Second, the diameter of graph $G'_s$ for each $s$ can be higher than the diameter of $G$, and thus it is not suitable for distributed implementation.

To deal with the first issue, we modify $G'_s$ into
a \textit{cut-equivalent} graph by adding new terminal sets along $N_G(U_s)$. For any vertex sets $A,B \subseteq V$, $\kappa_G(A,B)$ is the size of an $(A,B)$-vertex mincut.
\begin{lemma} \label{lem:cut-equivalent terminal graph}
Given $G'_s$, define $G''_s$ as follows. First, remove $t$ from $G'_s$. Then, for each vertex $u \in N(U_s)$, add a new vertex $y$ along with an edge $(u,y)$. Denote $Y$ as the set of new vertices. Then, every $(s,t)$-cut in $G'_s$ is an $(s,Y)$-cut in $G''_s$ and vice ver sa. In particular, $\kappa_{G'_s}(s,t) = \kappa_{G''_s}(s,Y)$.
\end{lemma}
\begin{proof}
If $S$ is an $(s,t)$-separator in $G'_s$, then denote a vertex cut $(L,S,R)$ in $G'_s$ where $s \in L, t \in R$. Since $N_{G'_s}(t) \subseteq S \cup R$,   every vertex in $Y$ in $G''_s$ does not have an edge to $L$. Therefore, $(L, S, (R \cup Y) - \{t\})$ is a vertex cut in $G''_s$. If $S$ is an $(s,Y)$-separator in $G''_s$, then the same separator must be an $(s,t)$-separator in $G'_s$ by contracting all $Y$ into $t$.
\end{proof}

By \Cref{lem:cut-equivalent terminal graph}, we can run the graph $G''_s$ in the distributed setting because each new vertex $y$ can be simulated inside the corresponding vertex $u$ in its edge $(u,y)$.

To deal with the second issue, we classify the connected component $U_s$ into small or large. Let $b$ be a parameter to be determined. If $|U_s| \geq b$, then there are at most $O(n/b)$ such components. If  $|U_s| \leq b$, then the graph $G''_s$ can have many nodes because $N_G(U_s)$ can still be large. Our goal is to reduce $N_G(U_s)$ to a set of size $O(|U_s|)$ while preserving the connectivity.


\begin{lemma} [Cluster Sparsification] \label{lem:sparsify by MM}
    Given $G''_s$,  denote $Z := N_{G''_s}(s) \cap N_{G''_s}(Y)$ as the common neighbors between $s$ and $Y$. There is an $\tilde O(1)$-round algorithm that returns a vertex set $D \subseteq N_G(U_s)$ satisfying the following property. Define $H_s$ as the graph $G''_s$ after removing $Z \cup (N_{G}(U_s) - D)$ and isolated vertices in $Y$, and denote $Y'$ to be the remaining nodes in $Y$. Then, $\kappa_{G''_s}(s,Y) = \kappa_{H_s}(s,Y') + |Z|$. If $W$ is an $(s,Y')$-mincut in $H_s$,  then $W \cup Z$ is an $(s,Y)$-mincut in $G''_s$.  Furthermore, $|V(H_s)| = O(|U_s|)$.
\end{lemma}

We prove \Cref{lem:sparsify by MM} in \Cref{sec:sparsification}. We are now ready to state the distributed algorithm in \congest model, and prove \Cref{lem:isolating cut congest}.

\paragraph{Algorithm (\congest).} The inputs consist of graph $G = (V,E)$, an independent set $T \subseteq V$ of size at least $2$, and an integer $b$ to be determined.
\begin{enumerate} [noitemsep]
    \item Encode each $t \in T$ as a binary string of length $\ceil{\log_2|T|}$. For each $i \leq  \ceil{\log_2|T|}$, define       $A_i :=  \{ t \in T \colon i^{\text{th}} \text{bit of }  $t $ = 0 \}$ and   $B_i := T - A_i$.
    Compute $F_i := (A_i,B_i)$-vertex mincut.
    \item For each $s \in T$, compute a connected component containing $s$, denoted by $U_s$, in $G - \bigcup_iF_i$.
    \item For each $s \in T$,
    \begin{enumerate} [noitemsep]
        \item If $|U_s| \leq b$, then construct $G''_s$ and compute $H_s$ using \Cref{lem:sparsify by MM}. Compute an $(s,Y')$-min-separator in $H_s$.
        \item If $|U_s| > b$, compute an $(s,Y)$-min-separator in $G''_s$.
    \end{enumerate}
    \item Return the minimum separators found during the algorithm.
\end{enumerate}


\paragraph{Running Time.}  The first two steps can be implemented in $O( T_{\textbm}(n,D) \cdot \log |T|)$ rounds (\Cref{lem:ST vc problem in matching}). In step (3a), we run $\tilde O(|V(H'_s)|)$-round maximum matching algorithm by \cite{AhmadiKO18} to compute $(s,Y')$-min-separator in $H'_s$. This steps takes $\tilde O(|V(H'_s)|) = \tilde O(|U_s|) = \tilde O(b)$ rounds. The first equality follows by \Cref{lem:sparsify by MM}. Step (3b) takes $O(\frac{n}{b} \cdot T_{\textbm}(n,D))$ rounds. This follows since we run a subgraph bipartite matching in time $O(T_{\textbm}(n,D))$ on each instance, and there are at most $O(n/b)$ instances. The total running time is $\tilde O(\frac{n}{b} \cdot T_{\textbm}(n,D) + b)$ rounds. By choosing $b = \tilde \Theta(\sqrt{n\cdot T_{\textbm}(n,D)})$, we get the desired running time.

\paragraph{Correctness.} Steps 1 and 2 are identical to the sequential algorithm. We now focus on Step 3. Fix a vertex $s \in T$. We prove that the algorithm returns an $(s,t)$-min-separator in $G_s$. By \Cref{lem:cut-equivalent terminal graph}, an $(s,Y)$-min-separator in $G''_s$ is also a $(s,t)$-min-separator in $G'_s$. Hence, if $|U_s| > b$, then we are done. We now prove for the case $|U_s| \leq b$. By \Cref{lem:sparsify by MM}, an $(s,Y')$-min-separator in $H'_s$ is also an $(s,Y)$-min-separator in $G'_s$, and we are done.





